Joint-MAE: 2D-3D Joint Masked Autoencoders for 3D Point Cloud Pre-training

Masked Autoencoders (MAE) have shown promising performance in self-supervised learning for both 2D and 3D computer vision. However, existing MAE-style methods can only learn from the data of a single modality, i.e., either images or point clouds, which neglect the implicit semantic and geometric correlation between 2D and 3D. In this paper, we explore how the 2D modality can benefit 3D masked autoencoding, and propose Joint-MAE, a 2D-3D joint MAE framework for self-supervised 3D point cloud pre-training. Joint-MAE randomly masks an input 3D point cloud and its projected 2D images, and then reconstructs the masked information of the two modalities. For better cross-modal interaction, we construct our JointMAE by two hierarchical 2D-3D embedding modules, a joint encoder, and a joint decoder with modal-shared and model-specific decoders. On top of this, we further introduce two cross-modal strategies to boost the 3D representation learning, which are local-aligned attention mechanisms for 2D-3D semantic cues, and a cross-reconstruction loss for 2D-3D geometric constraints. By our pre-training paradigm, Joint-MAE achieves superior performance on multiple downstream tasks, e.g., 92.4% accuracy for linear SVM on ModelNet40 and 86.07% accuracy on the hardest split of ScanObjectNN.

==> ablation.tex <==
\section{Ablation Study}
In this section, we conduct ablations to explore the effectiveness of different components in Joint-MAE. We utilize the final designed network as the baseline, and compare the linear SVM classification accuracy (\%) on ModelNet40~\cite{modelnet40}.

\subsection{Modal-specific Embedding Module and Decoder.}
On top of our final design, we conduct experiments with removing the modal-specific embedding modules and modal-shared decoder respectively. As reported in Table~\ref{block}, the absence of either modal-specific embedding module hurts the performance. Also, the modal-shared decoder well benefits the accuracy by providing complementary cross-modal information.
\begin{table}[h]
\vspace{0.1cm}
\centering
\small
\tabcaption{\textbf{Modal-specific Embedding Module and Joint Decoder}. `-' denotes the absence of the module, while `\checkmark' represents involved in.}
\vspace{-0.2cm}
\label{block}
	\begin{tabular}{ccccc}
	\toprule
            \multicolumn{2}{c}{\ Embed. Modules\ } &\multicolumn{2}{c}{Joint Decoder} &\makecell*[c]{\multirow{2}*{Acc. (\%)}}\\
		 \cmidrule(lr){1-2}  \cmidrule(lr){3-4}
		 \ \ \ 2D\ \ \  &3D &Modal-shared &Modal-specific &\\
		 \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
            \checkmark &\checkmark &\checkmark &\checkmark & \textbf{92.1} \\
	    \checkmark &-  &\checkmark  &\checkmark &91.2 \\
            - & \checkmark & \checkmark & \checkmark &91.4 \\
            \checkmark &\checkmark &- &\checkmark &91.8 \\
             %\vspace{0.1cm}\\
            % \rowcolor{blue!5}
	  \bottomrule
	\end{tabular}
\end{table}

\subsection{Local-aligned Attention.}
In Table~\ref{attn_abla}, we experiment different attention schemes for different cross-modal positions shown in Figure~\ref{attn}, i.e., 2D-3D and 3D-2D correlative tokens. We denote the local-aligned attention and the original attention as `Local' and `Global', respectively. The first row represents our Joint-MAE with local-aligned attention for all cross-modal positions. Compared with others, the local-aligned attention mechanism contributes to +0.5\% classification accuracy, indicating that the proposed methods can boost point cloud representation learning with 2D fine-grained semantic cues.

\begin{table}[h]
\vspace{0.1cm}
\centering
\small
\tabcaption{\textbf{Local-aligned Attention}. We utilize `Global’ and `Local’ to denote the standard global attention and local-aligned attention mechanism respectively. `2D-3D’ and `3D-2D’ denote the cross-modal positions during attention calculation.}
\label{attn_abla}
	\begin{tabular}{ccccc}
	\toprule
 \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ Attention Schemes\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ } &\makecell*[c]{\multirow{2}*{\ \ \ Acc. (\%)\ \ \ }} \\
 \cmidrule(lr){1-2} 
    \ \ \ \ \ \ \ 2D-3D\ \ \ \ \ \ \  &3D-2D & \\
		 \cmidrule(lr){1-1}  \cmidrule(lr){2-2} \cmidrule(lr){3-3}
            Global &Global &91.6 \vspace{2pt}\\
            Local &Global  &91.8 \vspace{2pt}\\
            Global &Local &92.0 \vspace{2pt}\\
            Local &Local &\textbf{92.1}\\
	  \bottomrule
	\end{tabular}
\vspace{-0.1cm}
\end{table}

\subsection{Cross-reconstruction Loss.}
In Table~\ref{loss_abla}, we explore the effectiveness and projection settings of the cross-reconstruction loss. As reported, the proposed cross-reconstruction loss contributes to at least +0.5\% on the classification performance. The comparison of the middle two rows reveals that projecting from multiple perspectives, which gives more geometric constraints, can benefit 3D point cloud pre-training. Also, the performance decay in the last row indicates that the rendering operation might introduce extra information which alleviates the effective supervision on the reconstructed 3D point cloud.

\begin{table}[h]
% \vspace{0.1cm}
\centering
\small
\tabcaption{\textbf{Loss function.} `View Num' denotes the view number of projections in the cross-reconstruction loss. `Render' denotes whether we conduct color rendering on the projected 2D depth maps.}
\label{loss_abla}
\vspace{-0.2cm}
	\begin{tabular}{cccc}
	\toprule
        \makecell*[c]{\multirow{2}*{\ \ \ \ Cross-Reconstruct.\ \ \ \ }} &\multicolumn{2}{c}{\ \ \ Proj. Settings\ \ \ } &\makecell*[c]{\multirow{2}*{\ \ Acc. (\%)\ \ }} \\
        \cmidrule(lr){2-3}
        &View Num. &Render & \\
		 \cmidrule(lr){1-1}  \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
            - &- &- & 91.1\\
            \checkmark &1 &- &91.6 \\
            \checkmark &4 &- &\textbf{92.1} \\
            \checkmark &4 &\checkmark &91.9 \\
	  \bottomrule
	\end{tabular}
\end{table}
% \end{minipage}
